HELP: Hardware-Adaptive Efficient Latency Prediction for NAS via Meta-Learning

For deployment, neural architecture search should be hardware-aware, in order to satisfy the device-specific constraints (e.g., memory usage, latency and energy consumption) and enhance the model efficiency. Existing methods on hardware-aware NAS collect a large number of samples (e.g., accuracy and latency) from a target device, either builds a lookup table or a latency estimator. However, such approach is impractical in real-world scenarios as there exist numerous devices with different hardware specifications, and collecting samples from such a large number of devices will require prohibitive computational and monetary cost. To overcome such limitations, we propose Hardware-adaptive Efficient Latency Predictor (HELP), which formulates the device-specific latency estimation problem as a meta-learning problem, such that we can estimate the latency of a model's performance for a given task on an unseen device with a few samples. To this end, we introduce novel hardware embeddings to embed any devices considering them as black-box functions that output latencies, and meta-learn the hardware-adaptive latency predictor in a device-dependent manner, using the hardware embeddings. We validate the proposed HELP for its latency estimation performance on unseen platforms, on which it achieves high estimation performance with as few as 10 measurement samples, outperforming all relevant baselines. We also validate end-to-end NAS frameworks using HELP against ones without it, and show that it largely reduces the total time cost of the base NAS method, in latency-constrained settings. Code is available at https://github.com/HayeonLee/HELP.

==> 1_Figure/acc_lat_trade_off.tex <==
\begin{figure*}[t!]
\centering
%\vspace{0.05in}
\includegraphics[width=\linewidth]{1_Figure_Raw/placeholder.pdf}
\caption{\small \textbf{Acc-Lat Trade off} }
\label{fig:trade}
\vspace{-0.1in}
\end{figure*}


==> 1_Figure/corr_num_sample.tex <==
% \begin{figure*}[t!]
% \centering
% \vspace{-0.15in}
% \includegraphics[width=0.9\linewidth]{1_Figure_Raw/num_sample.eps}
% \caption{\small \textbf{Effectiveness of Meta-Knowledge Transfer Dependent on The Number of Samples} }
% \label{fig:corr_num_sample}
% \vspace{-0.1in}
% \end{figure*}

\begin{wrapfigure}{r}{0.4\textwidth} 
 \vspace{-0.1in}
  \begin{center}
    \includegraphics[width=\linewidth]{1_Figure_Raw/num_sample.pdf}
    \caption{\small \textbf{Effectiveness of Meta-Knowledge Transfer Dependent on The Number of Samples} }
\label{fig:corr_num_sample}
  \end{center}
   \vspace{-0.1in}
\end{wrapfigure} 

% \begin{wrapfigure}{r}{0.4\textwidth} 
%  \vspace{-0.3in}
% \caption{A wrapped table going nicely inside the text.}\label{wrap-tab:1}

% \label{fig:size_meta_train}
%  \vspace{-0.3in}
% \end{wrapfigure} 


==> 1_Figure/e2e_nas_ofa.tex <==
\begin{figure*}[t!]
\centering
\vspace{-0.05in}
\includegraphics[width=0.9\textwidth]{1_Figure_Raw/e2e_nas_ofa.eps}
\caption{Comparison between searched architecture by HELP+OFA and other state-of-the-art NAS methods in MobileNet-based space.}
\label{fig:e2e_nas_ofa}
\vspace{-0.1in}
\end{figure*}

==> 2_Table/corr_fbnet.tex <==
\begin{table*}[t!]
	\caption{\small \textbf{Meta-Test: Correlation on Unseen Devices with Few-shot Samples (FBNet Search Space)} }%MetaD2A conducts amortized inference on unseen target datasets after meta-training on source database consisting of subsets of ImageNet-1K and architectures of NAS-Bench-201 search space. Meta-training time is 12.7/8.4 GPU hours for the generator/the predictor. For fair comparison, the parameters of searched architectures are trained on each dataset from scratch instead of transferring parameters from ImageNet. $T$ is the time to construct precomputed architecture database for each target. We report accuracies with $95\%$ confidence intervals. } %  45797/30152 GPU seconds
	\vspace{-0.15in}
	\small
	\begin{center}
     \resizebox{\linewidth}{!}{
	    \begin{tabular}{ll|c|c|ccc|ccc|c}
	   	\toprule
	   	\multicolumn{2}{c|}{\multirow{2}{*}{Method}} & 
	   	\multirow{2}{*}{Transfer}                     &
	   	Sample                                       & 
	   	\multicolumn{3}{c|}{Unseen Device}           &
	   	\multicolumn{3}{c|}{Unseen Platform}           \\
	                                                 &
	                                                 &
	                                                 &
	    (N)                                          &
	   	Titan                                        & 
	   	Xeon                                         & 
        Pixel3                                       & 
	   	Raspi4                                       &
	   	Eyeriss                                      &
	    FPGA                                         &
	   	Mean                                         \\
	   	\midrule
	   	\midrule
	   %	\multicolumn{1}{c|}{\multirow{6}{*}{FBNet}}  &
	   %	\multicolumn{1}{l|}{FLOPS}                  &
	   %	                                            &
	   %	                                            &
	   % -                                           &
	   %	x.xxx                                       &
	   %	x.xxx                                       &
	   % x.xxx                                       &
	   % x.xxx	   		   	                        &
	   % x.xxx                                       &
	   % x.xxx                                       &
	   % x.xxx                                       \\
	   %	\multicolumn{1}{l|}{Layer-wise Predictor}             &
	   %	                                            &
	   %	                                            &
	   % ?                                           &
	   %	x.xxx                                       &
	   %	x.xxx                                       &
	   % x.xxx                                       &
	   % x.xxx	   		   	                        &
	   % x.xxx                                       &
	   % x.xxx                                       &
	   % x.xxx                                       \\
	   % %\midrule
	   %	\multicolumn{1}{l|}{BRP-NAS~\citep{dudziak2020brp}}              &
	   %	                                            &
	   %	                                            &
	   % 10                                          &
	   %	0.266                                       &
	   %	0.318                                       &
	   % 0.366                                       &
	   % 0.303	   		   	                        &
	   % 0.315                                       &
	   % 0.346                                       &
	   % 0.319                                       \\
	   % \midrule
	   % \multicolumn{1}{l|}{BRP-NAS (+M.K.T)~\citep{dudziak2020brp}}                        &
	   %%	\multicolumn{1}{l|}{BRP-NAS~\citep{dudziak2020brp}}          &
	   %	                                            &
	   % \checkmark	                                &
	   % 10                                          &
	   %	x.xxx                                       &
	   %	0.xxx                                       &
	   % 0.xxx                                       &
	   % 0.xxx	   		   	                        &
	   % 0.xxx                                       &
	   % 0.xxx                                       &
	   % 0.xxx                                       \\
	   	\multicolumn{1}{l|}{MAML~\citep{finn2017model}}                  &
	   	                                            &
	   	\checkmark                                  &
	    10                                          &
	   	0.738                                       &
	   	0.544                                       &
	    0.576                                       &
	    0.568	   		   	                        &
	    0.602                                       &
	    0.541                                       &
	    0.595                                       \\
	                                               % &
	    \multicolumn{1}{l|}{Meta-SGD~\citep{li2017meta}}                 &
	   	                                            &
	   	\checkmark                                  &
	    10                                          &
	   	0.xxx                                       &
	   	0.xxx                                       &
	    0.786                                       &
	    0.844	   		   	                        &
	    0.831                                       &
	    0.882                                       &
	    0.850                                       \\
	   	\multicolumn{1}{l|}{ANP~\citep{kim2019atten}}                    &
	   	                                            &
	   	\checkmark                                  &
	    10                                          &
	   	0.888                                       &
	   	0.853                                       &
	    0.745                                       &
	    0.801	   		   	                        &
	    0.657                                       &
	    0.884                                       &
	    0.805                                       \\
	                                               % &
	   \midrule
	    \multicolumn{1}{l|}{\multirow{4}{*}{\textbf{HaNAS (Ours)}}}      &
	   	Amortization                                &
	   	\checkmark                                  &
	    10                                          &
	   	0.738                                       &
	   	0.546                                       &
	    0.577                                       &
	    0.568	   		   	                        &
	    0.604                                       &
	    0.539                                       &
	    0.596                                       \\
	    \multicolumn{1}{l|}{}                                            &
	   	+ HW-Condition                              &
	   	\checkmark                                  &
	    10                                          &
	   	0.957                                       &
	   	0.920                                       &
	    0.861                                       &
	    0.853	   		   	                        &
	    0.904                                       &
	    0.861                                       &
	    0.893                                      \\
	    \multicolumn{1}{l|}{}                                            &
	   	+ Few-Shot Adapt                            &
	   	\checkmark                                  &
	    10                                          &
	   	0.964                                       &
	   	\textbf{0.927}                              &
	    0.865                                       &
	    0.872	   		   	                        &
	    0.913                                       &
	    0.866                                       &
	    0.901                                        \\
        \multicolumn{1}{l|}{}                                            &
	   	+ $z$ Modulator                             &
	   	\checkmark                                  &
	    10                                          &
	   	\textbf{0.964}                              &
	   	0.925                                       &
	    \textbf{0.894}                              &
	    \textbf{0.885}	   		   	                &
	    \textbf{0.942}                              &
	    \textbf{0.889}                              &
	    \textbf{0.916}                             \\
	    %\midrule
	   	%\textbf{HaNAS (Ours) $\bm{\theta}_0^\tau$}                               &
	   	 %\multicolumn{1}{l|}{}                                                    &
	   	 %                                                   &
	   	%\checkmark                                          &
	    %3000                                                &
	   	%\textbf{0.933}&%\tiny{$\pm$0.00}}                      &
	   	%\textbf{0.946}&%\tiny{$\pm$0.00}}                      &
	   	%\textbf{0.951}&%\tiny{$\pm$0.00}}                      &
	   	%\textbf{0.973}&%\tiny{$\pm$0.00}}                      &
	   	%\textbf{0.981}&%\tiny{$\pm$0.00}}                      &
	   	%\textbf{0.993}&%\tiny{$\pm$0.00}}                      &
	   	%\textbf{0.963}\\%\tiny{$\pm$0.00}}                      \\
	   	\bottomrule
        \end{tabular}
	    }
	\end{center}
	\small
	\label{tbl:corr_fbnet}
	\vspace{-0.15in}
	
\end{table*}

==> 2_Table/end2end_nas.tex <==
\begin{table*}[t]
    \begin{center}
    \caption{\small End-to-End NAS Results} 
    \resizebox{\linewidth}{!}{
            \begin{tabular}{l|c|cccc|cccc}
            \toprule
            \centering
             \multicolumn{1}{c}{\multirow{2}{*}{Model}} & Const. & Storage & Sample    & Building Time & AWS Cost &Params & MACs & Latency & Accuracy \\
                            & (ms) &   Space (MB) & (N) & (Wall Clock)       & (\$) &(M)  &   (M)  & (ms) & (\%)    \\
            \midrule
            \midrule
            MobileNetV3-Large       & x  & x     & -    & -  & - & 5.4M   & 219M   & x & x    \\
            \midrule
            MnasNet-A3~\citep{tan2019mnasnet}   & x   &x    & 8k     & -   & - & 5.2M    & 403M  & todo & 76.7 \\
            Proxylessnas-mobile     & x  &x     & 5k    & -   & -   & x   & x      & x & 74.6     \\
            Efficientnet B0         & x  &x      & -     & -   & - & x   & x     & x & x    \\
            FBNet-C~\citep{wu2019fbnet}                 & x  &x     & -    & -    & -  & 5.5M   & 375M   & todo &  74.9      \\
            \midrule
            % MetaD2A~\cite{lee2021rapid}                            &x       & x             & x               & x       & x        & x               & x & x                   \\
        
        \multirow{4}{*}{OFA~\cite{cai2020once}} & -    & x     &5k?       & x     & x & 4.1M   & 79M      & todo     & 70.0    \\ 
                                                 & -    & x     &5k?       & x     & x  & 5.1M  & 113M      & todo     & 72.4    \\ 
                                                & -    & x     &5k?       & x     & x & 4.7M   & 166M      &  todo    & 73.9    \\ 
                                                & -    & x     &5k?       & x     & x & 5.8M   & 208M      & todo     & 75.6    \\ 

            \midrule
            \multirow{3}{*}{OFA + HaNAS}      & 70     & x     & 10      & x     &x  & 9.0M    & 238M      & 70    & 76.0   \\ 
                                              & 80     & x     & 10      & x     &x  & 8.5M    & 268M      & 93    & 76.5    \\
                                             & 100     & x     & 10      & x     &x   & 8.5M   & 319M      & 114   & 77.2   \\
            %\midrule
            %MobileNetV3                         & x             & x               & x       & x        & x               & x                      \\
            %x                                   & x             & x               & x       & x        & x               & x                      \\
            %x                                   & x             & x               & x       & x        & x               & x                    \\
            %x                                   & x             & x               & x       & x        & x               & x                    \\            
            %OFA~\cite{cai2020once}              & x               & x       & x        & x             & x               & x       \\
            %\textbf{OFA + HaNAS (Ours) 40ms}                 & x               & x       & x        & x             & x               & x       \\ 
            %\midrule
            %MobileNetV3                         & x             & x               & x       & x        & x               & x                      \\
            %x                                   & x             & x               & x       & x        & x               & x                      \\
            %x                                   & x             & x               & x       & x        & x               & x                    \\
            %x                                   & x             & x               & x       & x        & x               & x                    \\            
            %OFA~\cite{cai2020once}              & x               & x       & x        & x             & x               & x       \\
            %\textbf{OFA + HaNAS (Ours) 60ms}                 & x               & x       & x        & x             & x               & x       \\   
            %     \midrule                                           %sam                  %| %mac     %lat        %acc
        %   \multirow{3}{*}{MetaD2A + HaNAS}    & 70    & x     &10       & x     & x    & x      & 62.96     & 72.9    \\ 
        %                                       & 80     & x     &10       & x    & x     & x     & 83.7       & 72.9     \\
        %                                       & 100    & x      &10      & x     & x    & x     & 99.14      & 73.6     \\
            \bottomrule
            \end{tabular}
        }
    \end{center}
\end{table*}% \begin{table}[t]



==> 2_Table/knowledge.tex <==
\begin{minipage}[h!]{0.9\textwidth}
    \centering
	%\vspace{0.08in}
	\begin{minipage}{0.45\textwidth}
	    \vspace{0.05in}
		\centering 
		\small
     \resizebox{\linewidth}{!}{
	   % \begin{tabular}{l|c|c|cccccc|c}
	    \begin{tabular}{l|c|c|c}
	   	\toprule
	   %	\multicolumn{1}{c|}{\multirow{2}{*}{Search Space}}                                     &
	   	\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & 
	   	Knowledge                                    &
	   	Sample                                       & 
	   %	\multicolumn{6}{c|}{Spearman Correlation}    &
	   	                                            \\
	                                                 &
	    Transfer                                     &
	    (N)                                          &
	   %	Titan                                        & 
	   %	Xeon                                         & 
    %     Pixel3                                       & 
	   %	Raspi4                                       &
	   %	Eyeriss                                      &
	   % FPGA                                         &
	   	Mean                                         \\
	   	\midrule
	   	\midrule
	   	Task-Specific Model                         &
	   	                                            &
	    3000                                        &
	   %	0.856                                       &
	   %	0.791                                       &
	   % 0.926                                       &
	   % 0.953	   		   	                        &
	   % 0.960                                       &
	   % 0.980                                       &
	    0.911                                       \\
	   	Task-Specific Model                         &
	   	                                            &
	    3000                                        &
	   %	0.856                                       &
	   %	0.791                                       &
	   % 0.926                                       &
	   % 0.953	   		   	                        &
	   % 0.960                                       &
	   % 0.980                                       &
	    0.911                                       \\
	   	\textbf{HaNAS (Ours) $\bm{\theta}_0^\tau$}                               &
	   	\checkmark                                          &
	    3000                                                &
	   %	\textbf{0.967}                                      &
	   %	\textbf{0.933}                                      &
	   % \textbf{0.957}                                      &
	   % \textbf{0.975}	   		   	                        &
	   % \textbf{0.984}                                      &
	   % \textbf{0.997}                                      &
	    \textbf{0.968}                                      \\
	    \midrule
	   	Task-Specific Model                         &
	   	                                            &
	    3000                                        &
	   %	0.856                                       &
	   %	0.791                                       &
	   % 0.926                                       &
	   % 0.953	   		   	                        &
	   % 0.960                                       &
	   % 0.980                                       &
	    0.911                                       \\
	   	Task-Specific Model                         &
	   	                                            &
	    3000                                        &
	   %	0.856                                       &
	   %	0.791                                       &
	   % 0.926                                       &
	   % 0.953	   		   	                        &
	   % 0.960                                       &
	   % 0.980                                       &
	    0.911                                       \\
	   	\textbf{HaNAS (Ours) $\bm{\theta}_0^\tau$}                               &
	   	\checkmark                                          &
	    3000                                                &
	   %	\textbf{0.967}                                      &
	   %	\textbf{0.933}                                      &
	   % \textbf{0.957}                                      &
	   % \textbf{0.975}	   		   	                        &
	   % \textbf{0.984}                                      &
	   % \textbf{0.997}                                      &
	    \textbf{0.968}                                      \\
	    \midrule
	   	Task-Specific Model                         &
	   	                                            &
	    3000                                        &
	   %	0.856                                       &
	   %	0.791                                       &
	   % 0.926                                       &
	   % 0.953	   		   	                        &
	   % 0.960                                       &
	   % 0.980                                       &
	    0.911                                       \\
	   	Task-Specific Model                         &
	   	                                            &
	    3000                                        &
	   %	0.856                                       &
	   %	0.791                                       &
	   % 0.926                                       &
	   % 0.953	   		   	                        &
	   % 0.960                                       &
	   % 0.980                                       &
	    0.911                                       \\
	   	\textbf{HaNAS (Ours) $\bm{\theta}_0^\tau$}                               &
	   	\checkmark                                          &
	    3000                                                &
	   %	\textbf{0.967}                                      &
	   %	\textbf{0.933}                                      &
	   % \textbf{0.957}                                      &
	   % \textbf{0.975}	   		   	                        &
	   % \textbf{0.984}                                      &
	   % \textbf{0.997}                                      &
	    \textbf{0.968}                                      \\
	   	\bottomrule
        \end{tabular}
	    }
	\vspace{-0.12in}
	\captionof{table}{\small Ablation study on distributional shift.}\label{tbl:ood}
	\end{minipage}
	\begin{minipage}{0.5\textwidth}
		\vspace{-0.1in}
		\centering
		\includegraphics[height=4.5cm]{1_Figure_Raw/size_meta_training.pdf}\label{fig:mimg_tsne}
		\vspace{-0.2in}
		\captionof{figure}{\small T-SNE visualization of $\bs\theta$ and $\bs\theta \ast \E[\bz^\ts]$.}
		\label{fig:ood}
	\end{minipage}
	\vspace{-0.05in}
\end{minipage}

==> 2_Table/large_shot.tex <==
\begin{table*}[t!]
	\caption{\small \textbf{Effectiveness of Knowledge Transfer} }%MetaD2A conducts amortized inference on unseen target datasets after meta-training on source database consisting of subsets of ImageNet-1K and architectures of NAS-Bench-201 search space. Meta-training time is 12.7/8.4 GPU hours for the generator/the predictor. For fair comparison, the parameters of searched architectures are trained on each dataset from scratch instead of transferring parameters from ImageNet. $T$ is the time to construct precomputed architecture database for each target. We report accuracies with $95\%$ confidence intervals. } %  45797/30152 GPU seconds
	\vspace{-0.15in}
	\small
	\begin{center}
     \resizebox{\linewidth}{!}{
	    \begin{tabular}{l|c|c|ccc|ccc|c}
	   	\toprule
	   %	\multicolumn{1}{c|}{\multirow{2}{*}{Search Space}}                                     &
	   	\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & 
	   	Knowl.                                       &
	   	Sample                                       & 
	   	\multicolumn{3}{c|}{Unseen Device}           &
	   	\multicolumn{3}{c|}{Unseen Platform}           \\
	                                                 &
	    Transfer                                     &
	    (N)                                          &
	   	Titan                                        & 
	   	Xeon                                         & 
        Pixel3                                       & 
	   	Raspi4                                       &
	   	Eyeriss                                      &
	    FPGA                                         &
	   	Mean                                         \\
	   	\midrule
	   	\midrule
	   	Task-Specific Model                         &
	   	                                            &
	    3000                                        &
	   	0.557&%\tiny{$\pm$0.05}                       &
	   	0.911&%\tiny{$\pm$0.01}                       &
	    0.882&%\tiny{$\pm$0.01}                       &
	    0.912&%\tiny{$\pm$0.01}	   		   	        &
	    0.907&%\tiny{$\pm$0.02}                       &
	    0.933&%\tiny{$\pm$0.00}                       &
	    0.851\\%\tiny{$\pm$0.07}                       \\
	   	Init. of Meta-SGD~\citep{li2017meta}        &
	   	\checkmark                                  &
	    3000                                        &
	   	0.741&%\tiny{$\pm$0.00}                       &
	   	0.935&%\tiny{$\pm$0.00}                       &
	   	0.927&%\tiny{$\pm$0.00}                       &
	   	0.741&%\tiny{$\pm$0.00}                       &
	   	0.949&%\tiny{$\pm$0.00}                       &
	   	0.954&%\tiny{$\pm$0.00}                       &
	   	0.913\\%\tiny{$\pm$0.04}                       \\
	   	\textbf{HaNAS (Ours) $\bm{\theta}_0^\tau$}                               &
	   	\checkmark                                          &
	    3000                                                &
	   	\textbf{0.933}&%\tiny{$\pm$0.00}}                      &
	   	\textbf{0.946}&%\tiny{$\pm$0.00}}                      &
	   	\textbf{0.951}&%\tiny{$\pm$0.00}}                      &
	   	\textbf{0.973}&%\tiny{$\pm$0.00}}                      &
	   	\textbf{0.981}&%\tiny{$\pm$0.00}}                      &
	   	\textbf{0.993}&%\tiny{$\pm$0.00}}                      &
	   	\textbf{0.963}\\%\tiny{$\pm$0.00}}                      \\
	   	\bottomrule
        \end{tabular}
	    }
	\end{center}
	\small
	\label{tbl:large_shot}
	\vspace{-0.2in}
	
\end{table*}

==> 2_Table/nas_nasbench201.tex <==
% \begin{table}[t]
%     \begin{center}
%         \begin{tabular}{l|cccc}
%         \toprule
%         \centering
%         Model             & \# of Samples & Wall clock time & Latency & Accuracy \\
%         \midrule
%         MobileNetV2       & x             & x               & x       & x        \\
%         NASNet-A          & x             & x               & x       & x        \\
%         DARTS             & x             & x               & x       & x        \\
%         MnasNet           & x             & x               & x       & x        \\
%         FBNet-C           & x             & x               & x       & x        \\
%         ProxylessNAS      & x             & x               & x       & x        \\
%         MobileNetV3-Large & x             & x               & x       & x        \\ 
%         OFA               & x             & x               & x       & x        \\
%         \midrule
%         OFA +Ours         & x             & x               & x       & x        \\ 
%         \bottomrule
%         \end{tabular}
%     \end{center}
% \end{table}
\begin{table*}[t]
    \begin{center}
    \caption{\small \textbf{NAS Results on Unseen Devices (Meta-Test)} }
    \resizebox{\linewidth}{!}{
            \begin{tabular}{l|cccc|cccc}
            \toprule
            \centering
            Search Space      & \multicolumn{8}{c}{NAS-Bench-201}                                                                        \\
            \midrule
            Model             & \multicolumn{4}{c|}{BRP-NAS~\cite{dudziak2020brp}} & \multicolumn{4}{c}{HaNAS (Ours)} \\
            \midrule
                             & Sample & Time    & Latency & Accuracy & Sample & Time    & Latency & Accuracy \\
                             &        & (hours) & (ms)    & (\%)     &        & (hours) & (ms)    & (\%)  \\
            \midrule
            \midrule
            \multirow{3}{*}{Desktop GPU}        & x             & x               & x       & x        & x             & x               & x       & x \\
                                                & x             & x               & x       & x        & x             & x               & x       & x \\
                                                & x             & x               & x       & x        & x             & x               & x       & x \\
            \midrule
            \multirow{3}{*}{Desktop CPU}        & x             & x               & x       & x        & x             & x               & x       & x \\
                                                & x             & x               & x       & x        & x             & x               & x       & x \\
                                                & x             & x               & x       & x        & x             & x               & x       & x \\
            \midrule
            \multirow{3}{*}{Galaxy S21}         & x             & x               & x       & x        & x             & x               & x       & x \\ 
                                                & x             & x               & x       & x        & x             & x               & x       & x \\
                                                & x             & x               & x       & x        & x             & x               & x       & x \\
            \midrule
            \multirow{3}{*}{Google Pixel5}      & x             & x               & x       & x        & x             & x               & x       & x \\ 
                                                & x             & x               & x       & x        & x             & x               & x       & x \\
                                                & x             & x               & x       & x        & x             & x               & x       & x \\
            \bottomrule
            \end{tabular}
        }
    \end{center}
\end{table*}

==> 2_Table/nas_result.tex <==
\begin{table*}[t!]
	\caption{\small \textbf{NAS Results on Average of 9 Unseen Devices (Meta-Test)} }%MetaD2A conducts amortized inference on unseen target datasets after meta-training on source database consisting of subsets of ImageNet-1K and architectures of NAS-Bench-201 search space. Meta-training time is 12.7/8.4 GPU hours for the generator/the predictor. For fair comparison, the parameters of searched architectures are trained on each dataset from scratch instead of transferring parameters from ImageNet. $T$ is the time to construct precomputed architecture database for each target. We report accuracies with $95\%$ confidence intervals. } %  45797/30152 GPU seconds
	\vspace{-0.15in}
	\small
	\begin{center}
     \resizebox{\linewidth}{!}{
	    \begin{tabular}{cl|ccccc}
	   	\toprule
	   	\multirow{2}{*}{Search Space}                   & 
	   	\multicolumn{1}{c|}{\multirow{2}{*}{NAS Method}} & 
	   	\# of Samples                               & 
	   	Build Time                                  & 
	   	\multirow{2}{*}{Speed Up}                   &
    	Latency                                     & 
	   	Accuracy                                    \\ 
	   	                                            & 
	   	                                            & 
	   	(N)                                         & 
	   	(Sec)                                       & 
	   	                                            & 
        (ms)                                        & 
	   	(\%)                                        \\
	   	\midrule
	   	\midrule
%%%%%%%%%%%%%%%%%%%%%%%%   MobileNetV3  %%%%%%%%%%%%%%%%%%%%%%%%%
	   	\multirow{2}{*}{MobileNetV3}               &%~\citep{howard2019searching}                 &
	    OFA~\citep{cai2020once}                    &
	   	xxx                                        &
	   	xxxx                                       &
	    xxx$\times$                                &
	    x.xx	   		   	                       &
	   	x.xx\tiny$\pm$x.xx                        \\	   	
	   	                                           &
	   	\textbf{Ours}                              &
	   	\textbf{xx}                                &
	   	\textbf{xx}                                &
	   	x$\times$                                  &
	   	\textbf{x.xxx}	   		   	               &
	   	\textbf{xx.xx\tiny$\pm$x.xx}               \\
	   	\midrule
%%%%%%%%%%%%%%%%%%%%%%%%   Nas-Bench-201  %%%%%%%%%%%%%%%%%%%%%%%%%
	   	\multirow{2}{*}{NAS-Bench-201}             &%~\citep{howard2019searching}                 &
	    MetaD2A~\citep{lee2021rapid}               &
	   	xxx                                        &
	   	xxxx                                       &
	    xxx$\times$                                &
	    x.xx	   		   	                       &
	   	x.xx\tiny$\pm$x.xx                        \\	   	 	
	   	                                           &
	   	\textbf{Ours}                              &
	   	\textbf{xx}                                &
	   	\textbf{xx}                                &
	   	x$\times$                                  &
	   	\textbf{x.xxx}	   		   	               &
	   	\textbf{xx.xx\tiny$\pm$x.xx}               \\
	   	\midrule
%%%%%%%%%%%%%%%%%%%%%%%%   HAT  %%%%%%%%%%%%%%%%%%%%%%%%%
	   	\multirow{2}{*}{HAT (NLP)}             &%~\citep{howard2019searching}                 &
	    HAT~\cite{wang2020hat}                     &
	   	xxx                                        &
	   	xxxx                                      &
	    xxx$\times$                                &
	    x.xx	   		   	                       &
	   	x.xx\tiny$\pm$x.xx                        \\	   	  	
	   	                                           &
	   	\textbf{Ours}                              &
	   	\textbf{xx}                                &
	   	\textbf{xx}                                &
	   	x$\times$                                  &
	   	\textbf{x.xxx}	   		   	               &
	   	\textbf{xx.xx\tiny$\pm$x.xx}               \\
	   	\bottomrule
        \end{tabular}
	    }
	\end{center}
	\small
	\label{tbl:nas}
	\vspace{-0.15in}
	
\end{table*}

==> 2_Table/nas_time.tex <==

\begin{wraptable}{l}{8cm}
    \vspace{-0.2in}
    \centering
    \small{\caption{\small Speed improvement when combined with MetaD2A for rapid search on mobile phone (Pixel2)}} 
    \vspace{-0.05in}
    \resizebox{0.55\columnwidth}{!}{
            \vspace{-0.2in}
            \begin{tabular}{lcccc}
	   	\toprule
	   	
	   	\multicolumn{1}{c}{\multirow{2}{*}{Method}}        & 
	   	Sample                                             &
	   	Building Time                                      &
	   	Adaptation Cost                                    &
	    Speed Up	                                       \\
	   	                                                   &
	            	                                       &
	   (GPU Sec)	                                       &
	   (GPU Sec)	                                       &
	                                                       \\
	   	\midrule
	   	\midrule
        w/ BRP-NAS~\cite{dudziak2020brp}                    &
        900                                                 &
        1120                                                &
        1220                                                &
        $\times$1.0                                         \\
	    w/ HELP                                             &
        \textbf{10}                                                  &
        \textbf{25}                                                  &
        \textbf{125}                                                 &
        \textbf{$\times$9.76}                                        \\
	   	
	   	\bottomrule
	   	
	   	\end{tabular}
    }
    \vspace{-0.1in}
\end{wraptable}




==> 2_Table/suppl_ofa.tex <==
\FloatBarrier
\begin{table}[h]
    \begin{center}
    \caption{\small Comparison of NAS results on ImageNet using unseen platform device, Jetson AGX Xavier. By combining HELP with rapid NAS method such as OFA, we can obtain competitive latency-constrained architecture against architectures from other state-of-the-art NAS methods, reducing total NAS cost significantly.
    } 
    %\vspace{-0.1in}
    \label{tbl:suppl_ofa}
    \resizebox{\linewidth}{!}{
    
            \begin{tabular}{c|l|ccc|cc|cc}
             \toprule
             \centering
            %   \multicolumn{1}{c}{\multirow{2}{*}{Device}} & \multicolumn{1}{c|}{\multirow{2}{*}{Model}}  & MACs & Latency & Accuracy & \multicolumn{2}{c|}{Latency Model} & Total NAS Cost & Speed Up\\
              \multirow{2}{*}{Device} & \multicolumn{1}{c|}{\multirow{2}{*}{Model}}  & MACs & Latency & Accuracy & \multicolumn{2}{c|}{Latency Model} & Total NAS Cost & Speed Up\\
              & &   (M)  & (ms) & (\%) &Sample & Building Time  & (Wall Clock)&  \\
             \midrule
             \midrule
             
             
             &MobileNetV3-Large~\citep{howard2019searching}            
              & 219M   & 70.8 & 75.2   & -    & -    & - & -\\
             % \cdashline{2-10}\noalign{\vskip 0.75ex}
            % & Efficientnet B0               
            %& -     & -   & -    & 390M    & 44.4 & 77.1    \\
             Unseen Platform
            &MnasNet-A1~\citep{tan2019mnasnet}          
              & 312M  & 71.6 & 75.2  & 8k     & 24.9h     & 40,024.9h & 1.0$\times$\\
            
            
            Jetson AGX Xavier
            &ProxylessNAS-GPU~\citep{cai2018proxylessnas}          
              &  465M     & 82.6 & 75.1    & 5k    & 15.6h   & 515.6h &  78$\times$\\
            (Batch 16)
            & OFA+Layer-wise Pred.~\cite{cai2020once}     
               & 349M    & 69.2     & 75.8  &27k   & 84h & 84h  & 476$\times$\\
            \cdashline{2-9}\noalign{\vskip 0.75ex}
           
            & OFA + HELP (65ms)        
             & 243M      & 67.4    & 75.9  & \multirow{2}{*}{\textbf{10}}      & \multirow{2}{*}{\textbf{112s}}   &\multirow{2}{*}{\textbf{0.03h (112s)}} & \multirow{2}{*}{\textbf{1.3M$\times$}}\\ 
            & OFA + HELP (70ms)       
             & 279M      & 76.4    & 76.7   &       &   && \\

             \bottomrule
             \end{tabular}
            
            }
            
        \end{center}
    \vspace{-0.2in}
\end{table}% \begin{table}[t]
\FloatBarrier


==> 2_Table/suppl_plotform_corr.tex <==
\begin{table}[H]
    \begin{center}
    \caption{\small 
    } 
    %\vspace{-0.1in}
    \label{tbl:platform_corr}
    \resizebox{\linewidth}{!}{
    
            \begin{tabular}{l|cccccc}
             \toprule
             \centering
                    & GPU   & CPU   & Mobile    & Raspi4    & FPGA  & ASIC
            GPU     & 1     & 0.758 & 0.803     & 0.739     & 0.887 & 0.906
            CPU     & 0.758 & 1     & 0.892     & 0.844     & 0.943 & 0.586
            Mobile  & 0.803 & 0.892 & 1         & 0.808     & 0.924 & 0.624
            Raspi4
            FPGA
            ASIC
              

             \bottomrule
             \end{tabular}
            
            }
            
        \end{center}
    \vspace{-0.2in}
\end{table}% \begin{table}[t]

==> defs.tex <==

%\usepackage[numbers, sort&compress]{natbib}


\usepackage{amsmath, amssymb, bm, amsthm}
\usepackage{mathrsfs} 
\usepackage{mathtools}
\usepackage{thmtools}
\usepackage{enumitem}
\usepackage{subfigure}
\usepackage{color}
\usepackage{booktabs}
\usepackage{array}
\usepackage{tabularx, booktabs, multirow}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

%\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}


\usepackage[capitalize,nameinlink]{cleveref}


%\numberwithin{equation}{section}
%\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
%\newtheorem{defn}{Definition}[section]
\newtheorem{lem}{Lemma}[section]
%\newtheorem{cor}{Corollary}[section]
\newtheorem{cor}{Corollary}
%\newtheorem{prop}{Proposition}[section]
%\theoremstyle{definition}
%\newtheorem{algorithm}{Algorithm}[section]
%\newtheorem{example}{Example}[section]


\newcommand{\dee}{\mathrm{d}}
\newcommand{\grad}{\nabla}

\DeclareMathOperator{\ber}{Ber}
\DeclareMathOperator{\gammadist}{Gamma}
\DeclareMathOperator{\betadist}{Beta}
\DeclareMathOperator{\dir}{Dir}
%\DeclareMathOperator{\cat}{cat}
\DeclareMathOperator{\expon}{expon}
%\DeclareMathOperator{\unif}{unif}
%\DeclareMathOperator{\KL}{KL}
\DeclareMathOperator{\sgm}{sgm}
\DeclareMathOperator{\frob}{{F}}
\DeclareMathOperator{\softmax}{{softmax}}
\DeclareMathOperator{\var}{{Var}}
\DeclareMathOperator{\diag}{{diag}}
\DeclareMathOperator{\softplus}{{Softplus}}
\DeclareMathOperator{\pool}{{StatisticsPooling}}

\newcommand{\normal}{\mathcal{N}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\card}[1]{\vert {#1} \vert}
\newcommand{\distiid}{\overset{iid}{\dist}}
\newcommand{\distind}{\overset{ind}{\dist}}
\newcommand{\Indicator}[1]{\mathds{1}_{\{#1\}}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\defas}{\vcentcolon=}  % requires mathtools package
\newcommand{\iid}{i.i.d.}

\newcommand{\bepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\btheta}{{\boldsymbol{\theta}}}
\newcommand{\bTheta}{{\boldsymbol{\Theta}}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
%%\newcommand{\E}{{\mathbb{E}}}
\newcommand{\Real}{{\mathbb{R}}}
\newcommand{\calP}{{\mathcal{P}}}
\newtheorem{observation}{Observation}

\newcommand{\bzero}{\mathbf{0}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bof}{\mathbf{f}}
\newcommand{\bhy}{\widehat{\by}}
%\newcommand{\bW}{\mathbf{W}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bhW}{{\widehat{\bW}}}
\newcommand{\btW}{{\widetilde{\bW}}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bphi}{{\boldsymbol{\phi}}}
\newcommand{\bpi}{{\boldsymbol{\pi}}}
\newcommand{\noise}{{\boldsymbol{\varepsilon}}}

\newcommand{\ts}{{\tau}}

\newcommand{\bee}{\begin{eqnarray}}
\newcommand{\eee}{\end{eqnarray}}


